Measurement of hard double-parton interactions in W->lv+ 2 jet events at sqrt(s)=7 TeV with the ATLAS detector

The production of W bosons in association with two jets in proton-proton collisions at a centre-of-mass energy of sqrt(s)=7 TeV has been analysed for the presence of double-parton interactions using data corresponding to an integrated luminosity of 36/pb, collected with the ATLAS detector at the LHC. The fraction of events arising from double-parton interactions, fDP(D) has been measured through the momentum balance between the two jets and amounts to fDP(D) = 0.08 +- 0.01 (stat.) +- 0.02 (sys) for jets with transverse momentum PT > 20 GeV and rapidity |y|<2.8. This corresponds to a measurement of the effective area parameter for hard double-parton interactions of \sigma_eff = 15 +- 3 (stat.) +5 -3 (sys.) mb.

==> Makefile <==
LATEX    = latex
BIBTEX   = bibtex
DVIPS    = dvips

BASENAME = MPIPublication

default: testlatex

testlatex:
	latex  ${BASENAME}; \
	latex  ${BASENAME}; \
	bibtex ${BASENAME}; \
	latex  ${BASENAME}; \
	latex  ${BASENAME}
	dvips  ${BASENAME} -o ${BASENAME}.ps
	dvipdf -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress ${BASENAME}

testpdflatex:
	pdflatex  ${BASENAME}; \
	pdflatex  ${BASENAME}; \
	bibtex    ${BASENAME}; \
	pdflatex  ${BASENAME}; \
	pdflatex  ${BASENAME}

#
# standard Latex targets
#

%.dvi:	%.tex 
	$(LATEX) $<

%.bbl:	%.tex *.bib
	$(LATEX) $*
	$(BIBTEX) $*

%.ps:	%.dvi
	$(DVIPS) $< -o $@

%.pdf:	%.tex
	$(PDFLATEX) $<

.PHONY: clean

clean:
	#rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg 
	rm -f  *.aux *.log       *.blg *.brf *.cb *.ind *.idx *.ilg \
	      *.inx *.dvi *.toc *.out *~ ~* spellTmp 



==> bib.tex <==
\section*{References}
\begin{thebibliography}{99}
\makeatletter
\bibitem{Landshoff:1978fq}
 P.~V.~Landshoff and J.~C.~Polkinghorne,
 % ``Calorimeter triggers for hard collisions,''
  Phys.\ Rev.\  D {\bf 18},  3344 (1978).
\bibitem{Takagi:1979wn}
  F.~Takagi,
  %``Multiple production of 	quark jets off nuclei,''
  Phys.\ Rev.\ Lett.\ {\bf 43}, 1296 (1979) .
\bibitem{Goebel:1979mi}
  C.~Goebel, F.~Halzen and D.~M.~Scott,
  %``Double Drell-Yan annihilations In hadron collisions: novel tests of the constituent picture,''
  Phys.\ Rev.\  D {\bf 22},  2789 (1980).
\bibitem{Paver:1982yp}
  N.~Paver and D.~Treleani,
  %``Multi - quark scattering and large \pt~ jet production in hadronic collisions,''
  Nuovo Cim.\  A {\bf 70},  215 (1982).
%\cite{Mekhfi:1983az}
\bibitem{Mekhfi:1983az}
  M.~Mekhfi,
  %``Multiparton processes: an application to double Drell-Yan,''
  Phys.\ Rev.\  D {\bf 32},  2371 (1985).    
%\cite{Humpert:1983fy}
\bibitem{Humpert:1983fy}
  B.~Humpert,
  %``The production of gauge boson pairs by $\bar{p}p$ colliders,''
  Phys.\ Lett.\  B {\bf 135},  179 (1984).
\bibitem{Humpert:1984ay}
  B.~Humpert and R.~Odorico,
  %``Multiparton scattering and QCD radiation as sources of four jet events,''
  Phys.\ Lett.\  B {\bf 154},   211 (1985).
\bibitem{Ametller:1985tp}
  L.~Ametller, N.~Paver and D.~Treleani,
  %``Possible signature of multiple parton interactions in collider four jet events,''
  Phys.\ Lett.\  B {\bf 169},   289 (1986).
\bibitem{Halzen:1986ue}
  F.~Halzen, P.~Hoyer and W.~J.~Stirling,
  %``Evidence for multiple parton interactions from the observation of multi-muon events in Drell-Yan experiments,''
  Phys.\ Lett.\  B {\bf 188},  375-378 (1987).
\bibitem{Godbole:1989ti}
  R.~M.~Godbole, S.~Gupta and J.~Lindfors,
  %``Double parton scattering contribution to W+jets,''
  Z.\ Phys.\  C {\bf 47}, 69-74 (1990).
\bibitem{Mekhfi:1985dv}
  M.~Mekhfi,
 % ``Correlations in color and spin in multiparton processes,''
  Phys.\ Rev.\  D {\bf 32},  2380 (1985) .
\bibitem{Shelest:1982dg}
  V.~P.~Shelest, A.~M.~Snigirev and G.~M.~Zinovev,
  %``The multiparton distribution equations in QCD,''
  Phys.\ Lett.\  B {\bf 113},  325 (1982).
\bibitem{Tompkins:2011bv}
  ATLAS Collaboration,
  %``Measurement of the inelastic proton-proton cross-section at $\sqrt{s} =7$ TeV with the ATLAS detector,''  
Nat. Commun. 2,  463 (2011).
\bibitem{Antchev:2011vs}
  G.~Antchev \textit{et al.}, TOTEM Collaboration
  %``First measurement of the total proton-proton cross section at the LHC energy of $\sqrt{s} =7$ TeV,''  
  [arXiv:1110.1395 [hep-ex]].
\bibitem{Akesson:1986iv}
 T.~Akesson \textit{et al.}, AFS Collaboration, 
%``Double parton scattering in $pp$ collisions at $\sqrt{s}$ = 63\;GeV,''
  Z.\ Phys.\  C {\bf 34}, 163 (1987).
\bibitem{Alitti:1991rd}
J.~Alitti \textit{et al.}, UA2 Collaboration, 
%``A Study of multi-jet events at the CERN $\bar{p}p$ collider and a search for double parton scattering,''
  Phys.\ Lett.\  B {\bf 268},  145-154 (1991).
\bibitem{Abe:1993rv}
F.~Abe \textit{et al.}, CDF Collaboration, 
%``Study of four jet events and evidence for double parton interactions in $p\bar{p}$ collisions at $\sqrt{s} = 1.8\;$TeV,''
  Phys.\ Rev.\  D {\bf 47},  4857-4871 (1993) .
\bibitem{Abe:1997xk}
F.~Abe \textit{et al.}, CDF Collaboration, 
% ``Double parton scattering in $\bar{p}p$ collisions at $\sqrt{s}=1.8\;$TeV,''
  Phys.\ Rev.\  D {\bf 56},  3811-3832 (1997).
\bibitem{Abazov:2009gc}
V.~Abazov \textit{et al.}, D0 Collaboration, 
%``Double parton interactions in photon+3 jet events in $\bar{p}p$ collisions $\sqrt{s}$=1.96 TeV,''
  Phys.\ Rev.\  D {\bf 81}, 052012 (2010).
\bibitem{Calucci:1997uw}
  G.~Calucci and D.~Treleani,
  %``Double parton scatterings in high-energy hadronic collisions,''
  Nucl.\ Phys.\ Proc.\ Suppl.\  {\bf 71}, 392-399(1999).
\bibitem{Calucci:1999yz}
  G.~Calucci and D.~Treleani,
  %``Proton structure in transverse space and the effective cross-section,''
  Phys.\ Rev.\  D {\bf 60}, 054023 (1999).
\bibitem{Ryskin:2011kk}
  M.~G.~Ryskin and A.~M.~Snigirev,
  %``A fresh look at double parton scattering,''
  Phys.\ Rev.\  D {\bf 83}, 114047 (2011).
\bibitem{Kom:2011nu}
  C.~H.~Kom, A.~Kulesza and W.~J.~Stirling,
  %``Prospects for observation of double parton scattering with four-muon final states at LHCb,''
  [arXiv:1109.0309 [hep-ph]].
\bibitem{Gaunt:2009re}
  J.~R.~Gaunt and W.~J.~Stirling,
  %``Double parton distributions incorporating perturbative QCD evolution and momentum and quark number sum rules,''
  J. High Energy Phys. {\bf 1003}, 005 (2010).
%\bibitem{Gaunt:2011xd}
%  J.~R.~Gaunt, W.~J.~Stirling,
 % ``Double parton scattering singularity in one-loop integrals,''
 % J. High Energy Phys. {\bf 1106 } (2011)  048.
\bibitem{Diehl:2011tt}
  M.~Diehl and A.~Schafer,
 % ``Theoretical considerations on multiparton interactions in QCD,''
  Phys.\ Lett.\  B {\bf 698},   389-402(2011).
\bibitem{Drees:1996rw}
  M.~Drees and T.~Han,
  %``Signals for double parton scattering at the Fermilab Tevatron,''
  Phys.\ Rev.\ Lett.\  {\bf 77}, 4142-4145 (1996).
\bibitem{DelFabbro:1999tf}
  A.~Del Fabbro and D.~Treleani,
  %``A double parton scattering background to Higgs boson production at the LHC,''
  Phys.\ Rev.\  D {\bf 61}, 077502 (2000).
\bibitem{Kulesza:1999zh}
  A.~Kulesza and W.~J.~Stirling,
  %``Like-sign $W$ boson production at the LHC as a probe of double parton scattering,''
  Phys.\ Lett.\  B {\bf 475}, 168-175 (2000).
\bibitem{DelFabbro:2002pw}
  A.~Del Fabbro and D.~Treleani,
 % ``Double parton scatterings in $b$ quark pairs production at the CERN LHC,''
  Phys.\ Rev.\  D {\bf 66}, 074012 (2002).
\bibitem{Hussein:2006xr}
  M.~Y.~Hussein,
  %``A double parton scattering background to associated $WH$ and $ZH$ production at the LHC,''
  Nucl.\ Phys.\ Proc.\ Suppl.\  {\bf 174}, 55-58 (2007).
\bibitem{Maina:2009vx}
  E.~Maina,
  %``Multiple parton interactions, $\bar{t}t$ and $W$ + 4j production at the LHC,''
  J. High Energy Phys. {\bf 0904}, 098 (2009).
\bibitem{Maina:2009sj}
  E.~Maina,
  %``Multiple parton interactions in $Z$+4j, $W^{\pm} W^{\pm}$ + 0/2j and $W^{+} W^{-}$ + 2j production at the LHC,''
  J. High Energy Phys. {\bf 0909}, 081 (2009).
\bibitem{Berger:2009cm}
  E.~L.~Berger, C.~B.~Jackson and G.~Shaughnessy,
  %``Characteristics and estimates of double parton scattering at the Large Hadron Collider,''
  Phys.\ Rev.\ D {\bf 81}, 014014 (2010).
\bibitem{Gaunt:2010pi}
  J.~R.~Gaunt \textit{et al.},
  %``Same-sign $W$ pair production as a probe of double parton scattering at the LHC,''
  Eur.\ Phys.\ J.\  C {\bf 69}, 53-65 (2010).
\bibitem{Maina:2010vh}
  E.~Maina,
  %``Multiple parton interactions in $Z$+ jets production at the LHC. A comparison of factorized and non-factorized double parton distribution functions,''
  J. High Energy Phys. {\bf 1101}, 061 (2011).
\bibitem{ATLAS}
ATLAS Collaboration,
 %``The ATLAS Experiment at the CERN Large Hadron Collider,''
  JINST {\bf 3} (2008) S08003.
%\bibitem{Domdey:2009bg}
 % S.~Domdey, H.~J.~Pirner, U.~A.~Wiedemann,
  %``Testing the scale dependence of the scale factor $\Delta_{\rm{eff}}$ in double dijet production at the LHC,''
 % Eur.\ Phys.\ J.\  C {\bf 65}, (2010)  153-162.
\bibitem{Blok1}
B.~Blok \textit{et al.}, 
 %``pQCD physics of multiparton interactions,''
  Eur.\ Phys.\ J.\  C {\bf 72}, 1963 (2012).
\bibitem{Blok2}
B.~Blok \textit{et al.}, 
 %``The Four jet production at LHC and Tevatron in QCD,''
  Phys.\ Rev.\  D {\bf 83}, 071501 (2011).
\bibitem{Gaunt1}
J.~R.~Gaunt \textit{et al.},
 %``Probing double parton scattering with leptonic final states at the LHC,''
[arXiv:1110.1174v1 [hep-ex]].
\bibitem{Gaunt3}
J.~R.~Gaunt and W.~J.~Stirling,
 %``Single and Double Perturbative Splitting Diagrams in Double Parton Scattering,''
 [arXiv:1202.3056v1 [hep-ex]].
\bibitem{WjetsXS} 
ATLAS Collaboration, 
%``Study of jets produced in association with a W boson in $pp$ collisions at $\sqrt{s}$ = 7 TeV with the ATLAS detector,'' 
Phys.\ Rev.\ D {\bf 85}, 092002 (2012).
\bibitem{egamma}
ATLAS Collaboration,
%``egamma performance''  
Eur.\ Phys.\ J.\  C {\bf 72}, 1909 (2012).
\bibitem{muons}
ATLAS Collaboration,
%``muon performance''
cds.cern.ch/record/1281339/files/ATLAS-CONF-2010-064.pdf
\bibitem{antikt}
M.~Cacciari, G.~P.~Salam and G.~Soyez,
%``The anti-$k_t$ jet clustering algorithm,''
J. High Energy Phys. {\bf 0408}, 063 (2008).
\bibitem{LCCali1}
ATLAS Collaboration, 
%``Jet energy measurement with the ATLAS detector in proton-proton collisions at $\sqrt{s} = 7 TeV'',
Nucl. Instrum. Methods Phys. Res., Sect.\ A {\bf 545}, 803 (2005) 
\bibitem{jetpaper}
ATLAS Collaboration, 
%``Measurement of inclusive jet and dijet cross sections in proton-proton collisions at 7 TeV centre-of-mass energy with the ATLAS detector'',
CERN-PH-EP-2011-191
%\bibitem{mc10} 
%  ATLAS Collaboration, ``New ATLAS event generator tunes to 2010 data,''
%ATL-PHYS-PUB-2011-008.
\bibitem{geant} 
 S. Agostinelli \textit{et al.},
% ``\textsc{Geant4} - a simulation toolkit,''
Nucl. Instrum. Methods Phys. Res., Sect. A {\bf 506}, 250 (2003).
\bibitem{atlassim} 
ATLAS Collaboration, 
Eur.\ Phys.\ J.\  C {\bf 70}, 823 (2010).
\bibitem{CTEQ}
J.~Pumplin \textit{et al.}, 
%cteq author??
J. High Energy Phys. {\bf 0207}, 012 (2002).
\bibitem{alpgen} 
  M.~L.~Mangano \textit{et al.},
%  ``ALPGEN, a generator for hard multiparton processes in hadronic collisions,''
  J. High Energy Phys. {\bf 0307}, 001 (2003).
\bibitem{mlm} 
  J.~Alwall \textit{et al.}, 
%  ``Comparative study of various algorithms for the merging of parton showers and matrix elements in hadronic collisions''
  Eur.\ Phys.\ J.\  C {\bf 53}, 473 (2008).
\bibitem{herwig} 
  G.~Corcella \textit{et al.}, 
 % ``HERWIG 6: An event generator for hadron emission reactions with interfering gluons (including supersymmetric processes),''
  J. High Energy Phys. {\bf 0101}, 010 (2001).
\bibitem{jimmy} 
  J.~M.~Butterworth, J.~R.~Forshaw and M.~H.~Seymour,
  %``Multiparton interactions in photoproduction at HERA,''
  Z.\ Phys.\  C {\bf 72}, 637-646 (1996).
%\bibitem{mcanlo}
%S. Frixione and B.R. Webber, 
%``Matching NLO QCD computations and parton shower simulations,''
% J. High Energy Phys. 0206 (2002) 029 [hep-ph/0204244].
\bibitem{Sherpa} 
  T.~Gleisberg \textit{et al.},
%  ``Event generation with \textsc{Sherpa} 1.1,''
  J. High Energy Phys. {\bf 0902}, 007 (2009).
\bibitem{ckkw}
S.~Catani \textit{et al.},
%``QCD matrix elements + parton showers,''
  J. High Energy Phys. {\bf 0111}, 063 (2001).
\bibitem{pythia}
  T.~Sjostrand, S.~Mrenna and P.~Z.~Skands,
%  ``\textsc{Pythia} 6.4 Physics and Manual,''
  J. High Energy Phys. {\bf 0605}, 026 (2006).
\bibitem{powheg} 
  S.~Alioli \textit{et al.},
 % ``A general framework for implementing NLO calculations in shower Monte Carlo programs: the POWHEG BOX,''
  J. High Energy Phys. {\bf 1006}, 043 (2010).
\bibitem{mcanlo}
S. Frixione and B.R. Webber, 
%``Matching NLO QCD computations and parton shower simulations,''
 J. High Energy Phys. {\bf 0206}, 029 (2002).
\bibitem{RooUnfold} 
  T. Adye, 
%``Unfolding algorithms and tests using RooUnfold,'' 
[arXiv:1105.1160 [hep-ex]]. %\bibitem{lumi}
 %ATLAS Collaboration, ``Updated luminosity determination in $pp$ collisions at $\sqrt{s} =7$ TeV using the ATLAS detector,'' 
%ATLAS-CONF-2011-011.
\bibitem{Mangano:1988sq}
  M.~L.~Mangano,
 % ``Four jet production at the Tevatron collider,''
  Z.\ Phys.\  C {\bf 42}, 331 (1989).
\end{thebibliography}

